Numerical Integration and Dynamic Discretization in Heuristic Search Planning over Hybrid Domains

In this paper we look into the problem of planning over hybrid domains, where change can be both discrete and instantaneous, or continuous over time. In addition, it is required that each state on the trajectory induced by the execution of plans complies with a given set of global constraints. We approach the computation of plans for such domains as the problem of searching over a deterministic state model. In this model, some of the successor states are obtained by solving numerically the so-called initial value problem over a set of ordinary differential equations (ODE) given by the current plan prefix. These equations hold over time intervals whose duration is determined dynamically, according to whether zero crossing events take place for a set of invariant conditions. The resulting planner, FS+, incorporates these features together with effective heuristic guidance. FS+ does not impose any of the syntactic restrictions on process effects often found on the existing literature on Hybrid Planning. A key concept of our approach is that a clear separation is struck between planning and simulation time steps. The former is the time allowed to observe the evolution of a given dynamical system before committing to a future course of action, whilst the later is part of the model of the environment. FS+ is shown to be a robust planner over a diverse set of hybrid domains, taken from the existing literature on hybrid planning and systems.

==> experiments/Coverage.tex <==
&&& \multicolumn{3}{|c|}{\UPMurphi} & \multicolumn{3}{|c|}{\Dino} & \multicolumn{3}{|c|}{\ENHSP} & \multicolumn{3}{|c|}{\FSPlus$_{RK22,NV}$} & \multicolumn{3}{|c|}{\FSPlus$_{RK22}$} \\
 \hline  Domain & $\Delta_{max}$ &I&S&R&D&S&R&D&S&R&D&S&R&D&S&R&D\\
 \hline\multicolumn{1}{l|}{\textsc{Agile  Robot  0  5  Sec}} &0.5&100&82&1.11&14.46&82&21.10&18.68&100&10.55&8.5&100&0.47&7.0&100&8.00&6.5\\
 \multicolumn{1}{l|}{\textsc{Agile  Robot  1  Sec}} &1.0&100&0&n/a&n/a&0&n/a&n/a&0&n/a&n/a&100&0.14&10.0&97&0.89&7.4\\
 \multicolumn{1}{l|}{\textsc{Orbital  Rendezvous}} &100&5&1&35.92&99.00&0&n/a&n/a&5&0.36&2300.0&5&0.26&2900.0&5&0.46&2223.4\\
 \multicolumn{1}{l|}{\textsc{Convoys}} &1&6&2&2.58&18.50&3&99.31&15.33&6&4.21&11.7&6&3.57&12.3&6&4.78&11.6\\
 \multicolumn{1}{l|}{\textsc{Intercept}} &0.1&10&12&204.16&62.17&0&n/a&n/a&10&5.68&10.6&8&39.00&10.3&10&28.28&10.4\\
 \multicolumn{1}{l|}{\textsc{Intercept  1  Sec}} &1&10&0&n/a&n/a&0&n/a&n/a&0&n/a&n/a&0&n/a&n/a&10&85.93&10.5\\
 \multicolumn{1}{l|}{\textsc{Zermelo}} &100&100&0&n/a&n/a&0&n/a&n/a&92&6.16&2284.8&98&1.04&2225.5&94&1.23&2098.9\\
 \multicolumn{1}{l|}{\textsc{1D  Powered  Descent}} &1&20&10&209.64&26.10&18&47.25&40.33&20&1.99&31.4&19&2.75&31.1&16&1.80&28.5\\
 \multicolumn{1}{l|}{\textsc{Random  Orbital  Rendezvous}} &100&100&1&34.20&21.00&0&n/a&n/a&100&0.31&2104.0&100&0.09&2534.0&100&0.34&2059.8\\
 \multicolumn{1}{l|}{\textsc{Non  Linear  Car}} &1&8&10&1.78&15.00&10&176.00&16.80&8&0.55&10.4&8&1.68&10.5&8&0.72&10.2\\
 \multicolumn{1}{l|}{\textsc{Dino  Car}} &1&10&10&1.78&15.00&10&176.00&16.80&10&0.07&12.0&10&0.01&11.0&10&0.03&11.0\\


==> experiments/Coverage_Final.tex <==
&&& \multicolumn{2}{c|}{\UPMurphi} & \multicolumn{2}{c|}{\Dino} & \multicolumn{3}{c|}{\ENHSP} & \multicolumn{3}{c|}{\FSPlus$_{RK22,NV}$} & \multicolumn{3}{c}{\FSPlus$_{RK22}$} \\
 \hline  Domain & $\Delta_{max}$ &I&S&R&S&R&S&R&D&S&R&D&S&R&D\\

 \hline\multicolumn{1}{@{ }l@{ }|}{\textsc{1D  Powered  Descent}} &1&20&9&150.87&18&49.24&20&1.99&31.4&19&2.75&31.1&16&1.80&28.5\\
 \hline\multicolumn{1}{@{ }l@{ }|}{\textsc{Agile  Robot}} &0.5&100&82&0.94&0&TO&100&10.55&8.5&100&0.47&7.0&100&8.00&6.5\\
 \multicolumn{1}{@{ }l@{ }|}{} &1&100&0&TO&0&TO&0&TO&n/a&100&0.14&10.0&97&0.89&7.4\\
 \hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Convoys}} &1&6&4&0.89&3&99.31&6&4.21&11.7&6&3.57&12.3&6&4.78&11.6\\
 \hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Dino  Car}} &1&10&10&1.62&10&28.32&10&0.07&12.0&10&0.01&11.0&10&0.03&11.0\\
 \hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Intercept}} &0.1&10&10&226.99& \multicolumn{2}{c|@{ }}{Crashes}&10&5.68&10.6&8&39.00&10.3&10&28.28&10.4\\
 \multicolumn{1}{@{ }l@{ }|}{\textsc{}} &1&10&0&TO& \multicolumn{2}{c|@{ }}{Crashes} &0&TO&n/a&0&TO&n/a&10&85.93&10.5\\
 \hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Non  Linear  Car}} &1&8&8&179.72&0&TO&8&0.55&10.4&8&1.68&10.5&8&0.72&10.2\\
\hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Orb.  Rendezvous (L\"{o}hr)}} &100&5&1&35.92&\multicolumn{2}{c|@{ }}{Crashes}&5&0.36&2300.0&5&0.26&2900.0&5&0.46&2223.4\\
 \multicolumn{1}{@{ }r@{ }|}{\textsc{ (Random)}} &100&100&1&36.50&\multicolumn{2}{c|@{ }}{Crashes}&100&0.31&2104.0&100&0.09&2534.0&100&0.34&2059.8\\
 \hline
 \multicolumn{1}{@{ }l@{ }|}{\textsc{Zermelo}} &100&100& \multicolumn{2}{c|@{ }}{NS} & \multicolumn{2}{c|@{ }}{NS} &92&6.16&2284.8&98&1.04&2225.5&94&1.23&2098.9\\


==> experiments/Coverage_Full.tex <==
&&& \multicolumn{2}{|c|}{\UPMurphi} & \multicolumn{2}{|c|}{\Dino} & \multicolumn{3}{|c|}{\ENHSP} & \multicolumn{3}{|c|}{\FSPlus$_{RK22,NV}$} & \multicolumn{3}{|c|}{\FSPlus$_{RK22}$} \\
 \hline  Domain & $\Delta_{max}$ &I&S&R&S&R&S&R&D&S&R&D&S&R&D\\
 \hline\multicolumn{1}{l|}{\textsc{Agile  Robot  0  5  Sec}} &0.5&100&82&0.94&0&n/a&100&10.55&8.5&100&0.47&7.0&100&8.00&6.5\\
 \multicolumn{1}{l|}{\textsc{Agile  Robot  1  Sec}} &1.0&100&0&n/a&0&n/a&0&n/a&n/a&100&0.14&10.0&97&0.89&7.4\\
 \multicolumn{1}{l|}{\textsc{Orbital  Rendezvous}} &100&5&1&35.92&0&n/a&5&0.36&2300.0&5&0.26&2900.0&5&0.46&2223.4\\
 \multicolumn{1}{l|}{\textsc{Convoys}} &1&6&4&0.89&3&99.31&6&4.21&11.7&6&3.57&12.3&6&4.78&11.6\\
 \multicolumn{1}{l|}{\textsc{Intercept}} &0.1&10&10&246.70&0&n/a&10&5.68&10.6&8&39.00&10.3&10&28.28&10.4\\
 \multicolumn{1}{l|}{\textsc{Intercept  1  Sec}} &1&10&0&n/a&0&n/a&0&n/a&n/a&0&n/a&n/a&10&85.93&10.5\\
 \multicolumn{1}{l|}{\textsc{Zermelo}} &100&100&0&n/a&0&n/a&92&6.16&2284.8&98&1.04&2225.5&94&1.23&2098.9\\
 \multicolumn{1}{l|}{\textsc{1D  Powered  Descent}} &1&20&9&150.87&18&49.24&20&1.99&31.4&19&2.75&31.1&16&1.80&28.5\\
 \multicolumn{1}{l|}{\textsc{Random  Orbital  Rendezvous}} &100&100&1&36.50&0&n/a&100&0.31&2104.0&100&0.09&2534.0&100&0.34&2059.8\\
 \multicolumn{1}{l|}{\textsc{Non  Linear  Car}} &1&8&8&179.72&0&n/a&8&0.55&10.4&8&1.68&10.5&8&0.72&10.2\\
 \multicolumn{1}{l|}{\textsc{Dino  Car}} &1&10&10&1.62&10&28.32&10&0.07&12.0&10&0.01&11.0&10&0.03&11.0\\
 \multicolumn{1}{l|}{\textsc{Solar  Rover  1  Sec}} &1&20&0&n/a&0&n/a&0&n/a&n/a&7&167.09&203.0&7&170.38&202.9\\
 \multicolumn{1}{l|}{\textsc{Solar  Rover  10  Sec}} &10&20&0&n/a&0&n/a&0&n/a&n/a&0&n/a&n/a&20&0.39&528.8\\
 \multicolumn{1}{l|}{\textsc{Solar  Rover  100  Sec}} &100&20&0&n/a&0&n/a&0&n/a&n/a&0&n/a&n/a&20&0.02&529.5\\


==> related_work.tex <==
\todo[inline]{Editing in progress: most of the text here was in the Introduction
	originally and has been pushed in here in a somewhat abrupt manner.}
A well--known approach to solve such problems originates in clasical Control 
Theory~\cite{ogata:control} and especifically, the research focused on the problem of
\emph{Trajectory Optimization}, that is, finding the control signal that results in the trajectory
that minimises a given cost function. This classical approach suffers of two main
critical limitations. First, there is the assumption that
the dynamics of the system being analysed are \emph{stationary}, that is, they do not change
over time as a side effect of the trajectory over the state space induced by the control signal.
Second, existing methods cannot be readily extended to verify that those trajectories satisfy
a given set of constraints. The response to this has coalesced over the last decade into the discipline of  \emph{Hybrid Control Theory}~\cite{johansson:04:hybrid_control,goebel:09:hybrid_dynamical_systems}, and
basic questions remain still open concerning the existence, uniqueness, and dependence on initial conditions and other parameters of solutions.

An alternative approach is the one pursued by the domain--independent automated planning community, 
in which \emph{plans}, the analogue of CT control signals, are sought by reasoning over a
\emph{domain} theory given in a general language, \PDDLplus~\cite{fox:pddl_plus}. This language allows us
to encode compactly domains with intricate time--varying dynamics, with its semantics
anchored on Hybrid Automata (\HA) theory~\cite{henzinger:00:hybrid_automata}. Each modality of the domain
dynamics, or \emph{mode}, corresponds
with an specific set of \ode's that describes the system dynamics from a given starting time and for a certain given \emph{duration} or as long as certain \textcolor{red}{invariant?} conditions are satisfied by system states. Transitions between
modes take place due to direct intervention on state variables via the application of \emph{instantaneous}
actions, or \emph{naturally} as state variables are changed by the \ode's associated with the current mode.

Somewhat orthogonal to the previous one is the approach followed by the path planning comunity~\cite{lavalle:06:planning}, that integrates CT, variational optimization and search 
over continuous state spaces. Plans are made up by patching together in sequence either 
continuous or discrete control signals, and trajectories following from such plans have to 
comply with geometrical constraints. On the other hand,
an in a way not too different from classical heuristic search, work on path planning has focused on
very specific problem domains, and while very general and effective search algorithms exist,
such as Kuffner \& LaValle's \shortcite{kuffner:00:rrt} \RRT~and its descendants, performance 
still generally relies on coming up, in an ad-hoc fashion, for a good heuristic that works in the domain of interest.

Research in the Automated Planning community has followed mainly three approaches. First, \emph{searching} explicitly for
plans~\cite{mcdermott:03:icaps}, with existing
systems built on top of existing well established classical planning explicit~\cite{hoffmann:03:metricff,lohr:12:mpc,coles:12:jair,coles:14:icaps} or symbolic~\cite{edelkamp:01:mips,dellapenna:12:ai} search techniques.
A second approach consists in compiling  the domain theory into a logical formula contained in some suitably chosen and expressive fragment of First Order Logic (\FOL), check its consistency via an off--the--shelf solver, and if consistent, decoding plans from its 
models~\cite{shin:05:tmlpsat,bryce:15:aaai,cashmore:16:icaps}\todo[inline]{Enrico: maybe rintanen here? Miquel: Maybe}. Alternatively, yet still very
much in line with this, hybrid planning as theorem--proving approach, recent work builds 
upon recent advances~\shortcite{frehse:11:cav} on verification tools for \HA~theory, compiling 
\PDDLplus~descriptions into an amenable input
for the model checker of choice~\cite{bogomolov:14:aaai} and if the existence of the plan is
confirmed, it is extracted from the symbolic representation of the set of reachable states.


The planner is not subject to the expressive limitations of past approaches that are
mostly limited to \ode~made up of \emph{polynomial}~\cite{bryce:15:aaai} or \emph{linear}~\cite{cashmore:16:icaps,bogomolov:14:aaai,shin:05:tmlpsat} \todo[inline]{Enrico: are you sure about cashmore's work here? I think the limitation there is on the fact that the functions should be derivable. I guess you can represent quite a general class of polynomials. Miquel: Let
	me double check.} expressions, relying
on the numerical integration of the~\ode~set associated with the current domain dynamics'\emph{mode}
in order to calculate successor states.
